AT-SNN: Adaptive Tokens for Vision Transformer on Spiking Neural Network

In the training and inference of spiking neural networks (SNNs), direct training and lightweight computation methods have been orthogonally developed, aimed at reducing power consumption. However, only a limited number of approaches have applied these two mechanisms simultaneously and failed to fully leverage the advantages of SNN-based vision transformers (ViTs) since they were originally designed for convolutional neural networks (CNNs). In this paper, we propose AT-SNN designed to dynamically adjust the number of tokens processed during inference in SNN-based ViTs with direct training, wherein power consumption is proportional to the number of tokens. We first demonstrate the applicability of adaptive computation time (ACT), previously limited to RNNs and ViTs, to SNN-based ViTs, enhancing it to discard less informative spatial tokens selectively. Also, we propose a new token-merge mechanism that relies on the similarity of tokens, which further reduces the number of tokens while enhancing accuracy. We implement AT-SNN to Spikformer and show the effectiveness of AT-SNN in achieving high energy efficiency and accuracy compared to state-of-the-art approaches on the image classification tasks, CIFAR10, CIFAR-100, and TinyImageNet. For example, our approach uses up to 42.4% fewer tokens than the existing best-performing method on CIFAR-100, while conserving higher accuracy.

==> 03motivation.tex <==
\section{Motivation}


\subsection{Timestep level mask}

ACT~\ref{}와 A-ViT~\ref{}는 각각 single layer RNN과 vision transformer에서 정확도를 고려하여 DNN의 workload를 조절할 수 있는 adaptive computation time(ACT) 기법을 제안하였다.
%ACT는 입력에 따라 single layer RNN의 실행을 반복적으로 수행함으로써 정확도를 향상시키는 방법론을 제안하였다.
ACT는 입력 데이터에 따라 높은 정확도를 달성하기 위해 필요로 하는 workload가 다르다는 점에 착안하여 모든 입력 데이터에게 일괄적으로 동일한 workload를 할당하는 것이 아니라 정확도에 있어 더 중요하거나 복잡한(more informative) 입력에 더 많은 workload를 할당하고, 덜 중요하거나 단순한(less informative) 입력에 더 적은 workload를 할당함으로써 정확도는 유지하면서 DNN의 workload를 줄이는 방법론이다.
ACT를 활용한 기존의 연구들(A-ViT, SACT~\cite{})은 각 block들이 residual connection으로 연결되어 있기 때문에 매 block에서 유사한 feature를 유지할 수 있고, 이러한 동작 구조는 ACT와 유사한 구조를 지닌다는 것을 통해 RNN을 넘어 CNN과 ViT에도 ACT를 적용할 수 있음을 보여주었다.~\cite{}
SNN을 기반으로 하는 ViT~\cite{} 또한 각 block이 residual connection으로 연결되어 있기 때문에 block level의 A-ViT의 방법론을 적용할 수 있다.
하지만 ANN과 달리 SNN은 여러번의 timestep에 걸쳐 추론을 수행하는데, ACT를 timestep으로도 적용할 수 있는지에 대한 연구는 아직 없다.
우리는 다음 실험들을 통해 기존의 ACT에 timestep을 고려해 새롭게 재정의함으로써 SNN에도 ACT를 적용할 수 있다는 가능성을 보여준다.

\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth]{figures/motivation/AViTandSNN.pdf}
    \caption{Comparison between A-ViT and Ours}
    \label{fig:motivation_SNN}
\end{figure}

\begin{table}[]
\caption{Accuracy before and after shuffling}
\label{tab:shuffle_spike}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c}
\hline
Dataset       & Model            & T & Tokens      & Clean & Shuffled \\ \hline
Cifar-10      & Spikformer-4-384 & 4 & 8$\times$8  & 94.88 & 94.38    \\
Cifar-100     & Spikformer-4-384 & 4 & 8$\times$8  & 77.42 & 76.88    \\
Tiny-ImageNet & Spikformer-8-384 & 4 & 8$\times$8  & 65.23 & 64.33    \\ \hline
\end{tabular}%
}
\end{table}

Fig.~\ref{fig:motivation_SNN}는 ACT, A-ViT와 Ours의 동작 과정을 시각화한다.
A-ViT는 residual connection을 통해 서로 다른 weight의 block에서도 halting score를 축적할 수 있으며, 이렇게 축적한 halting score를 통해 각 token들의 연산을 중지할지를 결정한다.
우리도 하나의 timestep에 대해 동일한 방식으로 동작할 수 있다.
하지만 SNN은 timestep을 반복함으로써 추론을 수행하기 때문에 halting score를 계산함에 있어서도 timestep을 고려해 주어야 한다.
Tab.~\ref{tab:shuffle_spike}은 우리가 timestep level에서 halting score를 축적할 수 있는 단서를 제공한다.
Tab.~\ref{tab:shuffle_spike}은 각 block에서 서로 다른 timestep의 입력을 서로 섞어 추론한 결과를 보여준다.
서로 다른 timestep의 입력을 섞었음에도 불구하고 정확도는 크게 달라지지 않는데, 이는 timestep이 다르더라도 각 입력들이 유사한 feature를 지니고 있음을 암시한다.
즉, Fig.~\ref{fig:motivation_SNN}(c)에서 $x_{1,1} \approx x_{1,2}$가 성립함을 의미한다.
따라서 우리는 $t=2$의 두번째 block의 halting score를 계산할 때, $t=1$에서의 halting score를 축적할 수 있다.

\textbf{O1.} SNN의 timestep은 single layer RNN에서의 ACT와 그 형태가 유사하기 때문에 timestep level로 ACT를 확장할 수 있다.


\subsection{Temporal aware masking}

\begin{figure}[t!]
    \centering
    \subfloat[Temporal aware masking(TAM)]{\includegraphics[width=0.5\linewidth]{figures/motivation/temporal_mask_240728.pdf}}
    \subfloat[Accuracy gap between temporal aware masking(TAM) and random masking(RM) (TAM - RM)]{\begin{minipage}[b]{0.5\linewidth}\subfloat{\includegraphics[width=1\linewidth]{figures/motivation/motivation_mask_ts2_240728.pdf}}\phantomcaption\\
    \subfloat{\includegraphics[width=1\linewidth]{figures/motivation/motivation_mask_ts3_240728.pdf}}\\
    \subfloat{\includegraphics[width=1\linewidth]{figures/motivation/motivation_mask_ts4_240728.pdf}}
    \end{minipage}}
    \caption{temporal aware masking(TAM) \dhcmt{크기 등은 수정 예정입니다.} \dhcmt{실험 결과 RM보다 TAM의 firing ratio가 더 높은 것을 확인했습니다. TAM을 활용할 경우 RM보다 더 많은 spike로 더 많은 정보를 전달할 수 있습니다.}}
    \label{fig:motivation_mask}
\end{figure}


SNN은 ANN과 달리 timestep을 반복함으로써 accuracy를 높인다.
우리는 이때, 여러 timestep에 걸쳐 일괄적으로 동일한 token들을 없애는 것이 SNN의 accuracy를 더 높인다는 것을 확인하였다.
Fig.~\ref{fig:motivation_mask}(b)은 매 timestep에서 random한 token들을 mask하는 random mask(RM)와 첫 timestep에서 random하게 token을 mask하지만, 이후 timestep에서는 첫 timestep에서 mask되었던 token을 동일하게 mask하는 temporal aware mask(TAM)의 정확도 차이를 비교하였다.
가로축은 masked token의 수이며, 오른쪽으로 갈수록 더 적은 token이 mask된다.
대부분의 token이 mask되지 않았을 때에는 RM와 TAM의 정확도는 거의 유사하다.
하지만 token이 많이 mask될 수록 TAM가 RM보다 더 높은 정확도를 달성하는 것을 확인할 수 있다.
이는 많은 token들이 mask될 때에는 매 timestep에서 서로 다른 token을 mask하는 것보다 일괄적으로 같은 token을 mask하는 것이 더 높은 정확도를 달성할 수 있음을 의미한다.
이러한 현상은 SNN의 membrane potentials에 기인한 것으로, Fig.~\ref{fig:motivation_mask}(a)를 통해 설명할 수 있다.
SNN은 다음 block으로 spike를 fire하면서 정보를 전달하는데, fire를 위해서는 각 spiking neuron은 일정한 timestep동안 membrane potentials을 축적해야 한다.
이때, 만약 RM에 의해 매 timestep마다 서로 다른 token들이 mask되면, 여러 neuron이 membrane potentials을 축적할 충분한 timestep을 확보하지 못하게 된다.
반면, 동일한 수의 token을 mask하더라도 여러 timestep에 걸쳐 하나의 token을 일괄적으로 mask하면 mask되지 않은 token들이 membrane potentials을 축적할 충분한 시간을 확보할 수 있어 다음 block으로 정보를 전달할 수 있다.
이러한 차이는 token이 많이 mask될수록 커지고, masked token이 줄어들면 차이도 줄어든다.
우리는 이를 통해 다음과 같은 두번째 observation을 도출할 수 있다.

\textbf{O2.} 추론에 참여하는 token의 수가 적어질수록 매 timestep에서 무작위하게 token을 제거하는 것보다는 동일한 block에서는 동일한 token을 제거하는 것이 더 높은 정확도를 달성할 수 있다.

==> 03motivation_old_240803.tex <==
\section{Motivation}


\subsection{Timestep level mask}

\begin{table}[]
\caption{Accuracy before and after shuffling}
\label{tab:random_spike}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c}
\hline
Dataset       & Model            & T & Tokens      & Clean & Shuffled \\ \hline
Cifar-10      & Spikformer-4-384 & 4 & 8$\times$8  & 94.88 & 94.38    \\
Cifar-100     & Spikformer-4-384 & 4 & 8$\times$8  & 77.42 & 76.88    \\
Tiny-ImageNet & Spikformer-8-384 & 4 & 8$\times$8  & 65.23 & 64.33    \\ \hline
\end{tabular}%
}
\end{table}

ACT~\ref{}와 A-ViT~\ref{}는 각각 single layer RNN과 vision transformer에서 정확도를 고려하여 DNN의 workload를 조절할 수 있는 adaptive computation time(ACT) 기법을 제안하였다.
%ACT는 입력에 따라 single layer RNN의 실행을 반복적으로 수행함으로써 정확도를 향상시키는 방법론을 제안하였다.
ACT는 입력 데이터에 따라 높은 정확도를 달성하기 위해 필요로 하는 workload가 다르다는 점에 착안하여 모든 입력 데이터에게 일괄적으로 동일한 workload를 할당하는 것이 아니라 정확도에 있어 더 중요하거나 복잡한(more informative) 입력에 더 많은 workload를 할당하고, 덜 중요하거나 단순한(less informative) 입력에 더 적은 workload를 할당함으로써 정확도는 유지하면서 DNN의 workload를 줄이는 방법론이다.
ACT를 활용한 기존의 연구들(A-ViT, SACT~\cite{})은 각 block들이 residual connection으로 연결되어 있기 때문에 매 block에서 유사한 feature를 유지할 수 있고, 이러한 동작 구조는 ACT와 유사한 구조를 지닌다는 것을 통해 RNN을 넘어 CNN과 ViT에도 ACT를 적용할 수 있음을 보여주었다.~\cite{}
SNN을 기반으로 하는 ViT~\cite{} 또한 각 block이 residual connection으로 연결되어 있기 때문에 block level의 A-ViT의 방법론을 적용할 수 있다.
하지만 ANN과 달리 SNN은 여러번의 timestep에 걸쳐 추론을 수행하는데, ACT를 timestep으로도 적용할 수 있는지에 대한 연구는 아직 없다.
우리는 다음 실험들을 통해 기존의 ACT에 timestep을 고려해 새롭게 재정의함으로써 SNN에도 ACT를 적용할 수 있다는 가능성을 보여준다.

\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth]{figures/motivation/RNNandSNN.pdf}
    \caption{Comparison between RNN and SNN}
    \label{fig:motivation_SNN}
\end{figure}

Fig.~\ref{fig:motivation_SNN}는 RNN에서의 ACT와 SNN의 동작 과정 중 하나의 block에서의 입력과 출력을 보여준다.
ACT와 SNN은 그 동작과정이 매우 유사한데, 특히 RNN에 ACT를 적용함으로써 반복적으로 추론을 수행하는 것은 SNN에서 여러 timestep에 걸쳐 추론을 수행하는 방식과 거의 동일한 구조를 띈다.
ACT와 SNN 모두 동일한 block에 대해 입력을 반복적으로 수행하며, ACT는 hidden state에 따라, SNN은 membrane potentials에 따라 반복 추론의 결과값이 달라진다.
유일하게 다른 점은 ACT의 경우 입력에 $\delta_{n}$을 추가함으로써 앞선 입력과 매우 유사하지만, 앞선 입력과는 다른 입력 벡터를 생성해 입력한다.
따라서 $x \approx x + \delta_{1} \approx ... \approx x + \delta_{n}$이 성립한다.
반면 SNN에서는 $t$-th timestep에서는 앞선 block 및 앞선 timestep의 영향을 받은 $x_{t}$가 입력된다는 것이다.
우리는 각 timestep에서의 입력이 다른 정도를 확인해보기 위해 동일한 block에서 서로 다른 timestep의 입력을 무작위로 섞어 정확도를 측정하였다.
Tab.~\ref{tab:random_spike}은 각 block에서 서로 다른 timestep의 입력을 무작위로 섞어 추론했을 때의 정확도를 측정한 것이다.
결과는 서로 다른 timestep에서의 입력을 무작위로 섞었음에도 불구하고 정확도는 섞지 않았을 때와 거의 차이가 없음을 보여주며, 이는 동일한 block에서의 입력과 출력은 서로 다른 timestep이라고 하더라도 유사하다는 것을 강하게 암시한다. (최근의 연구~\cite{}들은 이러한 경향성을 보고 하고 있다.)
따라서 우리는 SNN에서의 timestep이 RNN에서의 ACT와 유사하게 동일한 block에 대해 $x_{1} \approx x_{2} \approx ... \approx x_{T}$를 성립한다고 할 수 있다.
이러한 실험을 통해 우리는 다음과 같은 Observation을 도출할 수 있다.

\textbf{O1.} SNN의 timestep은 single layer RNN에서의 ACT와 그 형태가 유사하기 때문에 timestep level로 ACT를 확장할 수 있다.


\subsection{Temporal aware masking}

\begin{figure*}[t!]
    \centering
    \subfloat[Temporal aware masking(TAM)]{\includegraphics[width=0.5\linewidth]{figures/motivation/temporal_mask_240728.pdf}}
    \subfloat[Accuracy gap between temporal aware masking(TAM) and random masking(RM) (TAM - RM)]{\begin{minipage}[b]{0.5\linewidth}\subfloat{\includegraphics[width=1\linewidth]{figures/motivation/motivation_mask_ts2_240728.pdf}}\phantomcaption\\
    \subfloat{\includegraphics[width=1\linewidth]{figures/motivation/motivation_mask_ts3_240728.pdf}}\\
    \subfloat{\includegraphics[width=1\linewidth]{figures/motivation/motivation_mask_ts4_240728.pdf}}
    \end{minipage}}
    \caption{temporal aware masking(TAM) \dhcmt{크기 등은 수정 예정입니다.}}
    \label{fig:motivation_mask}
\end{figure*}


SNN은 ANN과 달리 timestep을 반복함으로써 accuracy를 높인다.
우리는 이때, 여러 timestep에 걸쳐 일괄적으로 동일한 token들을 없애는 것이 SNN의 accuracy를 더 높인다는 것을 확인하였다.
Fig.~\ref{fig:motivation_mask}(b)은 매 timestep에서 random한 token들을 mask하는 random mask(RM)와 첫 timestep에서 random하게 token을 mask하지만, 이후 timestep에서는 첫 timestep에서 mask되었던 token을 동일하게 mask하는 temporal aware mask(TAM)의 정확도 차이를 비교하였다.
가로축은 masked token의 수이며, 오른쪽으로 갈수록 더 적은 token이 mask된다.
대부분의 token이 mask되지 않았을 때에는 RM와 TAM의 정확도는 거의 유사하다.
하지만 token이 많이 mask될 수록 TAM가 RM보다 더 높은 정확도를 달성하는 것을 확인할 수 있다.
이는 많은 token들이 mask될 때에는 매 timestep에서 서로 다른 token을 mask하는 것보다 일괄적으로 같은 token을 mask하는 것이 더 높은 정확도를 달성할 수 있음을 의미한다.
이러한 현상은 SNN의 membrane potentials에 기인한 것으로, Fig.~\ref{fig:motivation_mask}(a)를 통해 설명할 수 있다.
SNN은 다음 block으로 spike를 fire하면서 정보를 전달하는데, fire를 위해서는 각 spiking neuron은 일정한 timestep동안 membrane potentials을 축적해야 한다.
이때, 만약 RM에 의해 매 timestep마다 서로 다른 token들이 mask되면, 여러 neuron이 membrane potentials을 축적할 충분한 timestep을 확보하지 못하게 된다.
반면, 동일한 수의 token을 mask하더라도 여러 timestep에 걸쳐 하나의 token을 일괄적으로 mask하면 mask되지 않은 token들이 membrane potentials을 축적할 충분한 시간을 확보할 수 있어 다음 block으로 정보를 전달할 수 있다.
이러한 차이는 token이 많이 mask될수록 커지고, masked token이 줄어들면 차이도 줄어든다.
우리는 이를 통해 다음과 같은 두번째 observation을 도출할 수 있다.

\textbf{O2.} 추론에 참여하는 token의 수가 적어질수록 매 timestep에서 무작위하게 token을 제거하는 것보다는 동일한 block에서는 동일한 token을 제거하는 것이 더 높은 정확도를 달성할 수 있다.

==> 04_method_old_240802.tex <==
\section{\sys{}}


\subsection{Vision Transformer based on Spiking Neural Network}

We formulate a vision transformer network based on SNN~\cite{ZZH22,ZYZ23}
%\ym{Not in related work?}
as follows:

\begin{equation}
    f_{T}(x) = FC(\frac{1}{T} \sum^{T}_{t=1} \mathcal{B}^{L} \circ \mathcal{B}^{L-1} \circ \cdot \cdot \cdot \circ \mathcal{B}^{1} \circ \mathcal{S}(x)),
    \label{eq:gradient}
\end{equation}

$x \in \mathbb{R}^{T \times C \times H \times W}$는 입력 이미지, $T$는 timestep이다.
$\mathcal{S(\cdot)}$는 spike patch splitting module로, 입력 이미지를 $K^{0}$개의 token으로 나눈 뒤, embedding시켜 각 token별로 $\mathcal{T} \in \mathbb{R}^{K^{0} \times E}$을 생성한다.
$K^{l}$는 $l$-th block에 입력되기 전의 token의 수이고, $K^{0}$은 $\mathcal{S(\cdot)}$에 의해 나눠진 최초의 token의 개수이다. $E$는 embedding 차원의 수이다.
$\mathcal{B}(\cdot)$는 하나의 encoder block으로, Spike Self-Attention(SSA)과 MLP로 이루어져 있으며 이러한 block들은 model 전체에 총 $L$개 block이 존재한다.
\sys{}는 기존의 $\mathcal{B}(\cdot)$에 더해 후술할 token merge and mask module이 추가로 포함되어 있다.
$FC(\cdot)$는 fully-connected-layer이다.
spiking vision transformer는 $\mathcal{S(\cdot)}$에서 direct embedding method~\cite{WDL19}를 이용해 float 형태의 데이터들이 spike 형태로 변환한다.
최종적으로 모든 block을 통과한 모든 token들은 평균내어 $FC(\cdot)$에 입력된다.
$\mathcal{S}(x)$를 통과하면 입력 이미지 $x$는 여러개의 token으로 나뉘게 된다.
즉, $\mathcal{T}^{0,t}_{1:K} = \mathcal{S}(x)$이다.
이때, $t$번째 timestep, $l$번째 block에서 추론한 뒤의 token들의 집합을 $\mathcal{T}^{l, t}_{1:K^{l}}$ 이라고 하면 각 block에 대해 다음과 같이 나타낼 수 있다.

\begin{equation}
    \mathcal{T}^{l, t}_{1:K^{l}} = \mathcal{B}^{l}(\mathcal{T}^{l-1, t}_{1:K^{l-1}}),
    \label{eq:tokenes}
\end{equation}


\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/method/timestep_level_masking_240219.pdf}
    \caption{Block-level merging and masking example of \sys{}}
    \label{fig:model}
\end{figure*}


\subsection{Temporal-aware mask}

SNN을 기반으로 하는 Vision transformer는 각 block이 residual connection으로 연결되어 있기 때문에 A-ViT의 방법을 그대로 적용할 수 있다.
하지만 이러한 방법은 timestep에 대한 고려가 없기 때문에 효율적으로 token의 수를 줄일 수 없다.
따라서 우리는 O1에 기반하여 timestep을 고려해서 token을 효율적으로 조절하는 방법론을 제안한다.
이를 위해 우리는 \sys{}이 입력 이미지에 따라 token 수를 조절하기 위해 각 token별로 매 timestep과 매 block에서의 연산을 필요로 하는 정도를 나타내는 halting score를 산출한다.
$t$-th timestep, $l$-th block에서 $k$-th token의 halting score $h^{l, t}_{k}$는 다음과 같이 재정의할 수 있다.

\begin{equation}
    h^{l, t}_{k} = \sigma(\alpha \times \mathcal{T}^{l, t}_{k, 1} + \beta)
\end{equation}

$\sigma(\cdot)$는 logistic sigmoid function이고, $\alpha$와 $\beta$는 scaling factor이다.
sigmoid function에 의해 $0 \leq h^{l, t}_{k} \leq 1$이다.
우리는 token이 지니는 embedding vector의 첫번째 원소를 활용해 $h^{l, t}_{k}$를 계산한다.
halting score는 각 block에서의 output에 기반하여 계산되고, 각 token의 첫번째 원소를 통해 계산하기 때문에 block에 있는 MLP의 첫번째 node가 halting score를 학습한다.
우리는 각 timestep의 마지막 block인 $L$-th block에서 $h^{L, t}_{k}=1$로 하여 마지막 block에서 모든 token들이 멈추도록 강제한다.
반면, SNN의 특성상 timestep은 무한히 증가할 수 있기 때문에 학습에서 그 수치를 강제하지 않는다.

우리는 각 block과 timestep에서 halting score를 계산하고 이를 축적함으로써 여러 timestep과 block에 걸쳐 특정 timestep의 특정 token에게 특정 block에서의 연산이 필요한지를 평가한다.
우리는 A-ViT을 기반으로 동일한 timestep에서의 block 간의 halting score를 축적하면서, O1을 기반으로 동일한 block에서 timestep 간의 halting score도 축적할 수 있다.
따라서 $T'$번째 timestep과 $L'$번째 block에서 halting module $H_{k}(L', T')$를 다음과 같이 새롭게 정의할 수 있다.

\begin{gather}
    H_{k}(L', T') = \sum^{L'-1}_{l=1}\sum^{T'}_{t=1}h^{l, t}_{k} + \sum^{T'-1}_{t=1}h^{L', t}_{k}
    \label{eq:M_score}
\end{gather}

\sys{}는 $H_{k}(L', T')$를 통해 본인을 제외하고 같거나 작은 timestep과 block index에서의 halting score를 축적하며 $H_{k}(L', T') \geq 1 - \epsilon$인 token들의 결과를 0으로 변경함으로써 mask를 취한다.
만약 token $k$가 $L'$-th block, $T'$ timestep에서 mask 취해진다면, 해당 token은 추후 이어지는 모든 block($\geq L'$)과 timestep($\geq T'$)에서 $\mathcal{T}^{l, t}_{k} = 0$이 된다.

우리는 timestep을 고려하여 새롭게 정의한 halting score를 기반으로 \sys{}가 학습 과정에서 각 token에 따라 필요한 computation의 양을 결정할 수 있도록 하는 새로운 loss function을 제안한다.
\sys{}는 halting score를 timestep-level과 block-level로 축적하기 때문에 더 이른 timestep과 더 얕은 block에서 token이 mask될 경우 더 많은 computation을 절약할 수 있다.
이를 위해 $t$-th timestep에서 $k$-th token이 $H_{k}(L', T') \geq 1 - \epsilon$를 만족하는 block index인 $\mathcal{N}_{k}$와 $t$-th timestep과 $l$-th block에서 $k$-th token의 reminder인 $r^{l, t}_{k}$를 다음과 같이 정의한다.

\begin{equation}
    \mathcal{N}^{t}_{k} = \underset{l \leq L}{\mathrm{arg\,min}}\ H_{k}(l, t) \geq 1 - \epsilon,
\end{equation}

\begin{equation}
    r^{l, t}_{k} = 1 - H_{k}(l, t),
\end{equation}

$\epsilon$는 halting의 threshold를 결정하는 수로, 사전에 정의된 일정한 값을 가진다.
이를 기반으로 우리는 halting probability를 다음과 같이 정의할 수 있다.

\begin{equation}
    p^{l, t}_{k} = \Bigg\{ \begin{array}{l}
        h^{l, t}_{k}\text{ if }t = \{1, ..., T\}\text{ and }l < \mathcal{N}^{t}_{k}\\
        r^{l, t}_{k}\text{ if }t = \{1, ..., T\}\text{ and }l = \mathcal{N}^{t}_{k}\\
        0\text{ otherwise }
    \end{array}
\end{equation}

우리는 앞서 정의한 halting module 및 probability를 기반으로 \sys{}의 학습을 위해 다음과 같은 loss function들을 제안한다.
먼저 각 block 및 timestep에서의 output에 halting probability를 고려하여 누적 계산한다.
따라서 classification loss function $\mathcal{L}_{task}$을 다음과 같이 정의한다.

\begin{equation}
    \mathcal{L}_{task} = \mathcal{C}(FC(\frac{1}{T}\sum^{T}_{t=1}\sum^{L}_{l=1}\frac{1}{K^{l}}\sum^{K^{l}}_{k=1}\mathcal{T}^{l, t}_{k} \cdot p^{l, t}_{k}))
    \label{eq:cross_entrophy}
\end{equation}

$\mathcal{C}$는 cross-entropy loss이다.

그리고 앞서 정의했던 각 token의 $r_{k}, \mathcal{N}_{k}$을 통해 ponder loss $\mathcal{L}_{ponder}$를 다음과 같이 정의할 수 있다.

\begin{equation}
    \mathcal{L}_{ponder} = \frac{1}{TK^{L}} \sum_{t=1}^{T}\sum^{K^{L}}_{k=1}(t \times \mathcal{N}^{t}_{k} + r^{\mathcal{N}^{t}_{k}, t}_{k}),
\end{equation}


\begin{equation}
    \mathcal{L}_{overall} = \mathcal{L}_{task} + \delta_{p} \mathcal{L}_{ponder},
    \label{eq:final_loss}
\end{equation}

\subsection{Temporal-aware merge}

O2에서 확인했듯이 SNN은 ANN기반의 모델과 달리 각 block간의 정보를 전달하기 위해서는 spiking neuron이 특정 threshold까지 신호가 축적되지 않으면 안된다.
따라서 우리는 이러한 특성을 반영하기 위해 새로운 temporal-aware merge 기법을 제안한다.
기존의 연구들~\cite{}은 각 token의 feature 간의 유사성을 비교해 높은 유사도를 지니는 token들을 하나의 token으로 merge하였다.
\sys{}가 제안하는 temporal-aware merge도 feature 간의 유사성을 통해 token들을 merge하며, 다음과 같은 순서로 동작한다.

\begin{itemize}
    \item[1.] 첫번째 timestep에서 전체 token 중 짝수의 인덱스를 가지는 토큰을 A, 홀수의 인덱스를 가지는 토큰을 B group으로 나눈다.
    \item[2.] A그룹과 B그룹의 token들간의 cosine similarity를 계산한다.
    \item[3.] A그룹에서 유사도가 높은 $\gamma$개 token을 B그룹의 token과 매칭시킨다.
    \item[4.] 서로 매칭된 token들(다수의 A그룹 token과 하나의 B그룹 token)에서 A 그룹의 token들은 B그룹의 token에 정보를 축적하고 매칭된 A 그룹의 token들의 값은 0으로 변경한다.
    \item[5.] 이를 첫번째 timestep의 마지막 block까지 반복 수행한다.
    \item[6.] 이어지는 timestep에서는 동일한 block의 첫번째 timestep에서 매칭되어 소멸했던 A그룹에 속한 token을 대상으로 B그룹에서 유사도가 높은 토큰들을 재선택한다.
    \item[7.] 마찬가지로 A 그룹의 token들은 B그룹의 token에 정보를 축적하고 매칭된 A 그룹의 token들의 값은 0으로 변경하고, 이를 마지막 timestep까지 반복 수행한다.
\end{itemize}

첫번째 timestep에서는 A 그룹과 B 그룹의 token들 중 유사도가 가장 높은 쌍들을 가장 우선 merge한다.
하지만 첫 timestep 이후부터는 첫 timestep에서 제거된 token과 동일한 token이 제거되도록 강제하며, 이를 통해 우리는 동일한 block에서는 동일한 token들이 merge되어 사라지도록 한다.
temporal-aware merge는 정확도에 중요한 역할을 수행하는 token들이 merge에 의해 무작위하게 사라져 정보를 손실하는 경우를 최소화시킴으로써 정확도 손실을 막아줄 수 있다.
token간의 cosine simiarlity를 계산하기 때문에 추가적인 overhead가 필요하지만 연산과정에서의 에너지 소모량은 크지 않다.(detailed in Sec. VI)

